Generalized Reductions: Making any Hierarchical Clustering Fair and Balanced with Low Cost

Clustering is a fundamental building block of modern statistical analysis pipelines. Fair clustering has seen much attention from the machine learning community in recent years. We are some of the first to study fairness in the context of hierarchical clustering, after the results of Ahmadian et al. from NeurIPS in 2020. We evaluate our results using Dasgupta's cost function, perhaps one of the most prevalent theoretical metrics for hierarchical clustering evaluation. Our work vastly improves the previous $O(n^{5/6}poly\log(n))$ fair approximation for cost to a near polylogarithmic $O(n^\delta poly\log(n))$ fair approximation for any constant $\delta\in(0,1)$. This result establishes a cost-fairness tradeoff and extends to broader fairness constraints than the previous work. We also show how to alter existing hierarchical clusterings to guarantee fairness and cluster balance across any level in the hierarchy.

==> conclusions.tex <==
\section{Conclusions \& Potential Extensions}\label{sec:conclusions}
We place our work in the growing body of literature from the machine learning community focusing on fairness in clustering~\cite{ahmadian2020faircorr,backurs,bera2019fair,bera,brubach2020a,chakrabarti2021a,proportionalfairness,chierichetti2017fair,esmaeili2021fair,esmaeili2020probabilistic,kleindessner2,rosner}, addressing the relatively less well-studied~\cite{ahmadian2020fairhier,chhabra2020fair} \emph{hierarchical} fair clustering setting.  Our approach yields state-of-the-art $\cost$ approximations and is simpler and more explainable than prior methods~\citep{ahmadian2020fairhier,chhabra2020fair}. We believe this simplicity could lend itself to more general fairness guarantees as well as tighter cost approximations, and see this as a promising direction for future research.



==> fair.tex <==

\section{Fair Hierarchical Clustering}

We now discuss how to perform fair hierarchical clusterings using our rebalancing algorithms.


\input{stochastic}

\input{deterministic}

==> stochastic-old.tex <==
\subsection{Stochastically Fair Hierarchical Clustering}\label{sec:stochastic}

At this point, we almost have enough tools to solve stochastically fair hierarchical clustering. For this, however, we need a simple application of level abstraction (Definition~\ref{def:abstract}). We introduce $\treerm$ (Algorithm~\ref{alg:rebalancemerge}), which simply imposes a modified version of level abstraction on the bottom levels of the hierarchy. It is modified such that, instead of considering vertices between a certain depth, it effectively searches from leaves to the root, and stops when it hits a cluster of a certain size, parameterized by $t$. It then contracts these paths for each leaf, excluding the leaf itself. For ease of discussion, we simply call this \textit{modified level abstraction}. Distance for modified level abstraction is also defined as the maximum cluster size ratio of two points involved in contraction.

\begin{theorem}\label{thm:stoch}
Given a $\gamma$-approximation for $\cost$ and any $\delta\in (0,1)$, in the stochastic fairness setting, with $\frac{1}{1-\delta}\alpha_i \leq p_i(v) \leq \frac1{1+\delta}\beta_i$ for all $v\in V$ and $i\in [c]$, there is a $\frac{9(1-\delta)\gamma}{a\delta^2}\ln(cn)$-approximation for \sfhc{} where $a = \min_{i\in[c]}\alpha_i$. Additionally, the hierarchy is guaranteed to be $\frac16$-relatively balanced. On top of the operators of Theorem~\ref{thm:balance}, it only modifies the tree by applying one modified level abstraction operator with distance $\frac{3(1-\delta)}{a\delta^2}\ln(cn)$.
\end{theorem}

\codestochastic

If we assume $\alpha_i$ is constant for all $i\in[c]$, then this is an $O(\gamma\ln n)$ approximation. Note that the trade-off for $\delta$ is in the allowed $p_i(v)$ values as well as the resulting probability of success (though we assume $\delta$ is constant). As $\delta$ increases, so does our probability of success, but our bounds on $p_i(v)$ become tighter. We additionally briefly note that as the best $\gamma$ is known to be $O(\sqrt{\log n})$, this becomes a $O(\log^{3/2} n)$-approximation. It is quite impressive to achieve a still polylogarithmic approximation in the fairness context, as the current best known fair approximation (albeit, not with stochastic color assignment) is $poly(n)$~\cite{ahmadian2020fairhier}.



It might be tempting to suggest applying $\treerm$ to any existing hierarchy, as opposed to one that is $\frac16$-relatively balanced. However, we note that this process would not work on, for instance, a highly unbalanced tree where all internal nodes have at least one leaf-child. In that case, this algorithm would simply merge the bottom $\ln n$ vertices into a single cluster, thereby not guaranteeing fairness. This is why the rebalancing process is important.

Obviously, since we only apply modified level abstraction once, edge separation only happens once in the algorithm. Thus we only need to bound the abstraction distance. The largest cluster size is clearly going to be bounded of the height of the largest possible cluster at height $\log_3(\ln n)$.

\begin{proposition}\label{prop:stochdist}
In Algorithm~\ref{alg:rebalancemerge}, the modified level abstraction has distance at most $3t$.
\end{proposition}

\begin{proof}
Since the hierarchy is $\frac16$-relatively balanced, a parent can only be at most three times the size of a child. Therefore, since our modified level abstraction stops the first time a vertex $v$ has $n_T(v) \geq t$, that means its child $u$ had $n_T(u) < t$, so $n_T(v) \leq 3n_T(u) \leq 3t$. Note this is the largest vertex that can be a part of the contraction process.
\end{proof}

This should be enough to get our approximation, where our approximation factor clearly becomes $3t$ by the same reasoning as Lemma~\ref{lem:opabstract}. However, to get our fairness results, we need to use a Chernoff bound, thus we must guarantee that all internal nodes correspond to clusters of sufficiently large size. This too is easy to observe because of our loop end condition

\begin{proposition}\label{prop:stochsize}
In Algorithm~\ref{alg:rebalancemerge}, for any internal node $v$, $n_T(v) \geq t$.
\end{proposition}

\begin{proof}
The for loop merges every vertex that is sufficiently small into its parent. Thus, if we assume there is an internal node $v$ such that $n_T(v) < t$, it would actually be contracted into its parent during the process.
\end{proof}

Finally, we must show the fairness guarantee. Since fairness is union-closed, we only need to show this for the clusters at height 1 in the hierarchy. This comes from a Chernoff bound.

\begin{lemma}\label{lem:stochchernoff}
The resulting tree from Algorithm~\ref{alg:rebalancemerge} with $t = \frac{3(1-\delta)}{a\delta^2}\ln(cn)$ for $a = \min_{i\in[c]}\alpha_i$ and any $\delta>0$ is stochastically fair for given parameters $\alpha_i,\beta_i$ for all colors $i\in c$ with high probability.
\end{lemma}


\begin{proof}
Consider a vertex $v$ at height 1. By Proposition~\ref{prop:stochsize}, $n_T(v) \geq t = \frac{3(1-\delta)}{a\delta^2}\ln(cn)$. Fix some $i\in[c]$. Let $X_{iv} = |P_i\cap \leaves(v)|$ count the number of vertices of color $i$ in $\leaves(v)$. Note this is a sum of Bernoullis, so $\mathbb{E}[|X_{iv}|] = \sum_{u\in\clust(v)} p_i(u)$. Note tat we are given that $p_i(u) \geq \frac{1}{1-\delta}\alpha_i$ for all $u$. This gives us the following bounds from Proposition~\ref{prop:stochsize}:

\begin{align*}
\mathbb{E}[|X_{iv}|] \geq& \frac{3(1-\delta)}{a\delta^2}\ln (cn)\cdot \frac{1}{1-\delta}\alpha_i \geq \frac{3}{\delta^2}\ln (cn)
\\\mathbb{E}[|X_{iv}|]  \geq& \frac{1}{1-\delta}\alpha_i t
\\\mathbb{E}[|X_{iv}|]  \leq& \frac{1}{1+\delta}\beta_i t
\end{align*}

Then by a Chernoff bound with $\delta = \delta$:

\begin{align*}
P(|X_{iv} - \mathbb{E}[X_{iv}]| \geq \delta \mathbb{E}[X_{iv}]) \leq& 2\exp(-\mathbb{E}[X_{iv}]\delta^2/3)
\\=& 2\exp(-\frac{3}{\delta^2}\ln (cn)\delta^2/3)
\\=& \frac{2}{cn}
\end{align*}

Thus, with probability at least $1-\frac{2}{cn}$:

\begin{align*}
X_{iv} - \mathbb{E}[X_{iv}] \leq& \delta \mathbb{E}[X_{iv}]
\\X_{iv} \leq& (1+\delta)\mathbb{E}[X_{iv}]
\\\leq& (1+ \delta)\cdot \frac{1}{1+\delta} \beta_it
\\\leq& \beta_it
\end{align*}

In other words, the cluster $\leaves(v)$ satisfies the upper bound for color $i$. We also find that:

\begin{align*}
-X_{iv} + \mathbb{E}[X_{iv}] \geq& \delta \mathbb{E}[X_{iv}]
\\X_{iv} \geq& (1-\delta)\mathbb{E}[X_{iv}]
\\\geq& (1-\delta)\cdot \frac{1}{1+\delta} \alpha_it
\\\geq& \alpha_it
\end{align*}

Which means it also satisfies the upper bound. Take a union bound over all of the (maximum possible) $\frac{n}{t} = \frac{a\delta^2n}{3(1-\delta)\ln n}$ for all $c$ colors and we find that with probability at least $1 - \frac{2a\delta^2}{3(1-\delta)\ln n}$, all height 1 clusters must be fair, meaning the entire hierarchy must be fair by the union-bound property. Notice that all of these are constant except $n$, so this is with high probability.



\end{proof}
